Video2Sim2Real: Full-Stack Autonomous Dexterous Skill Acquisition from a Single Human Video

Human manipulation videos are a convenient and intuitive source for robot learning. However, directly transferring human dexterity to robots remains challenging due to perception errors and embodiment gap. To address this, we introduce Video2Sim2Real, a full-stack framework for autonomous skill acquisition from a single human manipulation video. Our framework first uses off-the-shelf foundation models to reconstruct a simulator-ready digital twin and extract robot and object motion priors. Rather than treating the extracted robot motion as a reliable reference throughout execution, our key idea is to recover and leverage the most fundamental sources of supervision from the demonstrated skill: We identify object-centric keyframes to optimize the corresponding robot configurations using object information from the simulator, and use these configurations as anchors that refine the robot motion such that it ultimately has the desired impact on the environment. To bridge the remaining sim-to-real gap, we introduce a sim-to-real strategy that decouples robustness to noisy and incomplete perception from variations in hand-object interaction dynamics. Specifically, we learn to recalibrate robot configurations from noisy real-world point clouds via IL, and leverage residual RL to perform local finger-level adaptations to ensure for robust and effective interactions. Finally, a collision-aware motion planning module enables spatial generalization to novel object configurations. Across several everyday manipulation tasks, Video2Sim2Real improves simulated task success, safety, and trajectory coherence over numerous baselines, and achieves better sim-to-real transfer than existing techniques. These results demonstrate a promising path toward autonomous dexterous skill acquisition from human videos.

==> appendices/E_residual_rl_mp.tex <==
\section{Residual RL for Sim-to-Real Transfer on Motion-Planning Trajectories}
\label{sec:Residual_RL_4_MP}
In addition to the observations used for single-trajectory tracking (i.e., $
\mathbf{o}_t =
\left[
\bar{\mathbf{q}}^{\mathrm{cur}}_t,\;
\bar{\mathbf{q}}_{t+1},\;
\mathbf{c}_t,\;
\Delta \mathbf{x}_t,\;
\Delta \theta_t
\right],
$), we also condition the observation on additional goal information to mitigate partial observability arising from trajectory divergence. Speficially, we include the initial 3D flow centroid of each trajectory, and the target one, and also the next-time flow centrpoid posiitons.


It should be noted that the training time is comparable to that of replicating a single human trajectory, as finger adaptation remains similar across all trajectories.


==> tables/jerkiness_table_arm_hand.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1.25pt}
\caption{\textbf{Arm and hand RMS jerk across refinement baselines.} Lower values indicate smoother command trajectories. Each task has Arm and Hand RMS jerk columns. The final Avg. group reports the average across all seven task-level means. Cells show mean $\pm$ sample std across seeds for baselines; Ours has one replay row per task. No entries are manually corrected.}
\label{tab:arm_hand_rms_jerk_no_manual}
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{@{} l c c c c c c c c c c c c c c c c @{}}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Apple Prep.}} & \multicolumn{2}{c}{\textbf{Peach Prep.}} & \multicolumn{2}{c}{\textbf{Steak Season.}} & \multicolumn{2}{c}{\textbf{Toy Rearr.}} & \multicolumn{2}{c}{\textbf{Tissue Box}} & \multicolumn{2}{c}{\textbf{Book Pass.}} & \multicolumn{2}{c}{\textbf{Tray Retr.}} & \multicolumn{2}{c}{\textbf{Avg.}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
 & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} \\
\midrule
Residual RL (Flow) & \mci{17.043}{10.208} & \mci{22.176}{16.010} & \mci{48.649}{21.869} & \mci{38.982}{23.652} & \mci{23.978}{10.860} & \mci{26.756}{10.736} & \mci{32.532}{24.950} & \mci{32.401}{24.587} & \mci{20.643}{9.443} & \mci{18.779}{3.325} & \mci{114.881}{57.488} & \mci{104.741}{71.100} & \mci{21.733}{4.381} & \mci{23.507}{1.110} & \mci{39.923}{34.713} & \mci{38.192}{30.119} \\
Residual RL (Flow + Aux) & \mci{27.104}{12.419} & \mci{33.869}{10.659} & \mci{69.648}{6.310} & \mci{95.008}{18.242} & \mci{43.636}{20.289} & \mci{46.807}{20.790} & \mci{28.720}{4.358} & \mci{27.440}{3.409} & \mci{33.837}{19.455} & \mci{22.213}{6.541} & \mci{181.780}{82.265} & \mci{131.850}{63.450} & \mci{25.494}{1.819} & \mci{30.668}{8.197} & \mci{58.603}{56.441} & \mci{55.408}{41.725} \\
Deep-mimic RL (Flow) & \mci{17.031}{6.490} & \mci{314.524}{194.161} & \mci{7.436}{3.625} & \secondbest{\mci{8.052}{8.175}} & \best{\mci{2.132}{1.178}} & \mci{8.426}{2.692} & \best{\mci{2.940}{1.708}} & \best{\mci{6.679}{3.085}} & \mci{4.857}{0.739} & \mci{11.874}{3.933} & \mci{7.566}{3.042} & \mci{6.992}{5.758} & \mci{129.924}{204.111} & \mci{255.311}{350.019} & \secondbest{\mci{24.555}{46.724}} & \mci{87.408}{136.014} \\
Deep-mimic RL (Flow + Aux) & \mci{173.126}{278.012} & \mci{202.673}{210.847} & \secondbest{\mci{7.321}{1.652}} & \best{\mci{5.464}{1.825}} & \secondbest{\mci{2.426}{0.913}} & \mci{8.678}{2.313} & \mci{12.401}{16.918} & \mci{197.901}{296.329} & \secondbest{\mci{3.435}{1.734}} & \secondbest{\mci{8.318}{1.280}} & \secondbest{\mci{4.202}{1.391}} & \secondbest{\mci{5.756}{1.509}} & \secondbest{\mci{5.890}{3.271}} & \mci{18.014}{11.749} & \mci{29.829}{63.274} & \mci{63.829}{93.322} \\
Pre-Contact Init (Flow) & \mci{761.718}{1275.098} & \mci{34.787}{7.608} & \mci{20.786}{2.153} & \mci{11.563}{6.505} & \mci{36.976}{9.782} & \mci{28.986}{8.490} & \mci{60.184}{29.968} & \mci{42.586}{17.338} & \mci{25.623}{27.822} & \mci{14.358}{16.966} & \mci{81.888}{57.548} & \mci{30.687}{12.170} & \mci{17.918}{7.749} & \secondbest{\mci{14.753}{10.812}} & \mci{143.585}{273.558} & \mci{25.389}{11.910} \\
Pre-Contact Init (Flow + Aux) & \mci{40.669}{19.137} & \mci{36.524}{16.367} & \mci{54.429}{7.793} & \mci{31.980}{2.320} & \mci{33.157}{12.670} & \mci{23.986}{6.268} & \mci{164.592}{187.589} & \mci{133.047}{146.977} & \mci{621.802}{1055.918} & \mci{10.310}{4.225} & \mci{242.401}{364.162} & \mci{36.367}{26.230} & \mci{26.260}{4.901} & \mci{21.562}{5.775} & \mci{169.044}{215.585} & \mci{41.968}{41.228} \\
Opt-Pre-Contact Init (Flow) & \secondbest{\mci{15.828}{5.009}} & \secondbest{\mci{12.111}{7.687}} & \mci{27.593}{4.817} & \mci{26.104}{4.015} & \mci{17.521}{3.109} & \mci{11.832}{1.782} & \mci{29.150}{0.875} & \mci{28.139}{4.926} & \mci{612.473}{1012.000} & \mci{21.659}{6.958} & \mci{625.472}{1038.066} & \mci{37.447}{23.724} & \mci{925.043}{895.925} & \mci{19.908}{17.176} & \mci{321.868}{387.087} & \mci{22.457}{9.104} \\
Opt-Pre-Contact Init (Flow + Aux) & \mci{38.240}{13.398} & \mci{28.917}{7.466} & \mci{31.017}{17.968} & \mci{29.137}{5.430} & \mci{27.967}{3.519} & \mci{19.092}{4.451} & \mci{40.200}{8.071} & \mci{48.108}{4.837} & \mci{10.967}{8.366} & \mci{9.470}{7.719} & \mci{937.894}{899.774} & \mci{34.364}{26.520} & \mci{1018.025}{861.695} & \mci{31.336}{16.650} & \mci{300.616}{463.389} & \mci{28.632}{12.097} \\
Object-only (Flow) & \mci{1410.388}{1225.379} & \best{\mci{8.725}{4.754}} & \mci{3057.588}{245.780} & \mci{11.369}{0.255} & \mci{4.809}{5.216} & \secondbest{\mci{8.264}{4.932}} & \mci{1106.043}{944.973} & \mci{12.904}{3.791} & \mci{883.106}{1489.059} & \mci{17.490}{3.138} & \mci{1064.386}{909.990} & \mci{13.574}{2.026} & \mci{544.880}{912.903} & \mci{23.563}{8.779} & \mci{1153.029}{954.355} & \secondbest{\mci{13.698}{5.354}} \\
Object-only (Flow + Aux) & \mci{323.554}{413.084} & \mci{21.164}{7.107} & \mci{595.318}{1000.819} & \mci{20.419}{6.671} & \mci{10.465}{8.078} & \mci{14.644}{5.232} & \mci{558.383}{939.635} & \mci{15.543}{8.902} & \mci{129.711}{196.062} & \mci{19.421}{2.983} & \mci{977.774}{1157.390} & \mci{15.714}{3.715} & \mci{1065.747}{899.920} & \mci{28.735}{9.585} & \mci{522.993}{401.045} & \mci{19.377}{4.871} \\
\textbf{Ours} & \best{10.285} & 16.402 & \best{4.086} & 8.349 & 4.222 & \best{3.076} & \secondbest{5.934} & \secondbest{11.570} & \best{0.447} & \best{0.122} & \best{0.417} & \best{0.122} & \best{0.251} & \best{0.140} & \best{\mci{3.663}{3.697}} & \best{\mci{5.683}{6.533}} \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/jerkiness_table_corrected.tex <==
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3.0pt}
% \caption{\textbf{Arm RMS jerk across refinement baselines.} Lower values indicate smoother trajectories. The final column reports the average across all seven tasks. Cells show mean $\pm$ sample std across seeds for baseline. %Ours has one replay row per task.
% }
% \label{tab:jerkiness_corrected}
% \resizebox{0.99\textwidth}{!}{%
% \begin{tabular}{@{} l c c c c c c c c @{}}
% \toprule
% \textbf{Method} & \textbf{Apple Prep.} & \textbf{Peach Prep.} & \textbf{Steak Season.} & \textbf{Toy Rearr.} & \textbf{Tissue Box} & \textbf{Book Pass.} & \textbf{Tray Retr.} & \textbf{Avg.} \\
% \midrule
% Residual RL (Flow) & \mci{17.043}{10.208} & \mci{48.649}{21.869} & \mci{23.978}{10.860} & \mci{32.532}{24.950} & \mci{20.643}{9.443} & \mci{114.881}{57.488} & \mci{21.733}{4.381} & \mci{39.923}{34.713} \\
% Residual RL (Flow + Aux) & \mci{27.104}{12.419} & \mci{69.648}{6.310} & \mci{43.636}{20.289} & \mci{28.720}{4.358} & \mci{33.837}{19.455} & \mci{181.780}{82.265} & \mci{25.494}{1.819} & \mci{58.603}{56.441} \\
% Deep-mimic RL (Flow) & \mci{17.031}{6.490} & \mci{7.436}{3.625} & \best{\mci{2.132}{1.178}} & \best{\mci{2.940}{1.708}} & \mci{4.857}{0.739} & \mci{7.566}{3.042} & \mci{129.924}{204.111} & \secondbest{\mci{24.555}{46.724}} \\
% Deep-mimic RL (Flow + Aux) & \mci{173.126}{278.012} & \secondbest{\mci{7.321}{1.652}} & \secondbest{\mci{2.426}{0.913}} & \mci{12.401}{16.918} & \secondbest{\mci{3.435}{1.734}} & \secondbest{\mci{4.202}{1.391}} & \secondbest{\mci{5.890}{3.271}} & \mci{29.829}{63.274} \\
% Pre-Contact Init (Flow) & \mci{761.718}{1275.098} & \mci{20.786}{2.153} & \mci{36.976}{9.782} & \mci{60.184}{29.968} & \mci{25.623}{27.822} & \mci{81.888}{57.548} & \mci{17.918}{7.749} & \mci{143.585}{273.558} \\
% Pre-Contact Init (Flow + Aux) & \mci{40.669}{19.137} & \mci{54.429}{7.793} & \mci{33.157}{12.670} & \mci{164.592}{187.589} & \mci{621.802}{1055.918} & \mci{242.401}{364.162} & \mci{26.260}{4.901} & \mci{169.044}{215.585} \\
% Opt-Pre-Contact Init (Flow) & \secondbest{\mci{15.828}{5.009}} & \mci{27.593}{4.817} & \mci{17.521}{3.109} & \mci{29.150}{0.875} & \mci{612.473}{1012.000} & \mci{625.472}{1038.066} & \mci{925.043}{895.925} & \mci{321.868}{387.087} \\
% Opt-Pre-Contact Init (Flow + Aux) & \mci{38.240}{13.398} & \mci{31.017}{17.968} & \mci{27.967}{3.519} & \mci{40.200}{8.071} & \mci{10.967}{8.366} & \mci{937.894}{899.774} & \mci{1018.025}{861.695} & \mci{300.616}{463.389} \\
% Object-only (Flow) & \mci{1410.388}{1225.379} & \mci{3057.588}{245.780} & \mci{4.809}{5.216} & \mci{1106.043}{944.973} & \mci{883.106}{1489.059} & \mci{1064.386}{909.990} & \mci{544.880}{912.903} & \mci{1153.029}{954.355} \\
% Object-only (Flow + Aux) & \mci{323.554}{413.084} & \mci{595.318}{1000.819} & \mci{10.465}{8.078} & \mci{558.383}{939.635} & \mci{129.711}{196.062} & \mci{977.774}{1157.390} & \mci{1065.747}{899.920} & \mci{522.993}{401.045} \\
% \midrule

% \textbf{Ours} & \best{10.285} & \best{4.086} & 4.222 & \secondbest{5.934} & \best{0.447} & \best{0.417} & \best{0.251} & \best{\mci{3.663}{3.697}} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1.25pt}
\caption{\textbf{Arm and hand RMS jerk across refinement baselines.} Lower values indicate smoother command trajectories. Each task has Arm and Hand RMS jerk columns. The final Avg. group reports the average across all seven task-level means. Cells show mean $\pm$ sample std across seeds for baselines。}
\label{tab:jerkiness_corrected}
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{@{} l c c c c c c c c c c c c c c c c @{}}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Apple Prep.}} & \multicolumn{2}{c}{\textbf{Peach Prep.}} & \multicolumn{2}{c}{\textbf{Steak Season.}} & \multicolumn{2}{c}{\textbf{Toy Rearr.}} & \multicolumn{2}{c}{\textbf{Tissue Box}} & \multicolumn{2}{c}{\textbf{Book Pass.}} & \multicolumn{2}{c}{\textbf{Tray Retr.}} & \multicolumn{2}{c}{\textbf{Avg.}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
 & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} & \textbf{Arm} & \textbf{Hand} \\
\midrule
Residual RL (Flow) & \mci{17.043}{10.208} & \mci{22.176}{16.010} & \mci{48.649}{21.869} & \mci{38.982}{23.652} & \mci{23.978}{10.860} & \mci{26.756}{10.736} & \mci{32.532}{24.950} & \mci{32.401}{24.587} & \mci{20.643}{9.443} & \mci{18.779}{3.325} & \mci{114.881}{57.488} & \mci{104.741}{71.100} & \mci{21.733}{4.381} & \mci{23.507}{1.110} & \mci{39.923}{34.713} & \mci{38.192}{30.119} \\
Residual RL (Flow + Aux) & \mci{27.104}{12.419} & \mci{33.869}{10.659} & \mci{69.648}{6.310} & \mci{95.008}{18.242} & \mci{43.636}{20.289} & \mci{46.807}{20.790} & \mci{28.720}{4.358} & \mci{27.440}{3.409} & \mci{33.837}{19.455} & \mci{22.213}{6.541} & \mci{181.780}{82.265} & \mci{131.850}{63.450} & \mci{25.494}{1.819} & \mci{30.668}{8.197} & \mci{58.603}{56.441} & \mci{55.408}{41.725} \\
Deep-mimic RL (Flow) & \mci{17.031}{6.490} & \mci{314.524}{194.161} & \mci{7.436}{3.625} & \secondbest{\mci{8.052}{8.175}} & \best{\mci{2.132}{1.178}} & \mci{8.426}{2.692} & \best{\mci{2.940}{1.708}} & \best{\mci{6.679}{3.085}} & \mci{4.857}{0.739} & \mci{11.874}{3.933} & \mci{7.566}{3.042} & \mci{6.992}{5.758} & \mci{129.924}{204.111} & \mci{255.311}{350.019} & \secondbest{\mci{24.555}{46.724}} & \mci{87.408}{136.014} \\
Deep-mimic RL (Flow + Aux) & \mci{173.126}{278.012} & \mci{202.673}{210.847} & \secondbest{\mci{7.321}{1.652}} & \best{\mci{5.464}{1.825}} & \secondbest{\mci{2.426}{0.913}} & \mci{8.678}{2.313} & \mci{12.401}{16.918} & \mci{197.901}{296.329} & \secondbest{\mci{3.435}{1.734}} & \secondbest{\mci{8.318}{1.280}} & \secondbest{\mci{4.202}{1.391}} & \secondbest{\mci{5.756}{1.509}} & \secondbest{\mci{5.890}{3.271}} & \mci{18.014}{11.749} & \mci{29.829}{63.274} & \mci{63.829}{93.322} \\
Pre-Contact Init (Flow) & \mci{761.718}{1275.098} & \mci{34.787}{7.608} & \mci{20.786}{2.153} & \mci{11.563}{6.505} & \mci{36.976}{9.782} & \mci{28.986}{8.490} & \mci{60.184}{29.968} & \mci{42.586}{17.338} & \mci{25.623}{27.822} & \mci{14.358}{16.966} & \mci{81.888}{57.548} & \mci{30.687}{12.170} & \mci{17.918}{7.749} & \secondbest{\mci{14.753}{10.812}} & \mci{143.585}{273.558} & \mci{25.389}{11.910} \\
Pre-Contact Init (Flow + Aux) & \mci{40.669}{19.137} & \mci{36.524}{16.367} & \mci{54.429}{7.793} & \mci{31.980}{2.320} & \mci{33.157}{12.670} & \mci{23.986}{6.268} & \mci{164.592}{187.589} & \mci{133.047}{146.977} & \mci{621.802}{1055.918} & \mci{10.310}{4.225} & \mci{242.401}{364.162} & \mci{36.367}{26.230} & \mci{26.260}{4.901} & \mci{21.562}{5.775} & \mci{169.044}{215.585} & \mci{41.968}{41.228} \\
Opt-Pre-Contact Init (Flow) & \secondbest{\mci{15.828}{5.009}} & \secondbest{\mci{12.111}{7.687}} & \mci{27.593}{4.817} & \mci{26.104}{4.015} & \mci{17.521}{3.109} & \mci{11.832}{1.782} & \mci{29.150}{0.875} & \mci{28.139}{4.926} & \mci{612.473}{1012.000} & \mci{21.659}{6.958} & \mci{625.472}{1038.066} & \mci{37.447}{23.724} & \mci{925.043}{895.925} & \mci{19.908}{17.176} & \mci{321.868}{387.087} & \mci{22.457}{9.104} \\
Opt-Pre-Contact Init (Flow + Aux) & \mci{38.240}{13.398} & \mci{28.917}{7.466} & \mci{31.017}{17.968} & \mci{29.137}{5.430} & \mci{27.967}{3.519} & \mci{19.092}{4.451} & \mci{40.200}{8.071} & \mci{48.108}{4.837} & \mci{10.967}{8.366} & \mci{9.470}{7.719} & \mci{937.894}{899.774} & \mci{34.364}{26.520} & \mci{1018.025}{861.695} & \mci{31.336}{16.650} & \mci{300.616}{463.389} & \mci{28.632}{12.097} \\
Object-only (Flow) & \mci{1410.388}{1225.379} & \best{\mci{8.725}{4.754}} & \mci{3057.588}{245.780} & \mci{11.369}{0.255} & \mci{4.809}{5.216} & \secondbest{\mci{8.264}{4.932}} & \mci{1106.043}{944.973} & \mci{12.904}{3.791} & \mci{883.106}{1489.059} & \mci{17.490}{3.138} & \mci{1064.386}{909.990} & \mci{13.574}{2.026} & \mci{544.880}{912.903} & \mci{23.563}{8.779} & \mci{1153.029}{954.355} & \secondbest{\mci{13.698}{5.354}} \\
Object-only (Flow + Aux) & \mci{323.554}{413.084} & \mci{21.164}{7.107} & \mci{595.318}{1000.819} & \mci{20.419}{6.671} & \mci{10.465}{8.078} & \mci{14.644}{5.232} & \mci{558.383}{939.635} & \mci{15.543}{8.902} & \mci{129.711}{196.062} & \mci{19.421}{2.983} & \mci{977.774}{1157.390} & \mci{15.714}{3.715} & \mci{1065.747}{899.920} & \mci{28.735}{9.585} & \mci{522.993}{401.045} & \mci{19.377}{4.871} \\
\textbf{Ours} & \best{10.285} & 16.402 & \best{4.086} & 8.349 & 4.222 & \best{3.076} & \secondbest{5.934} & \secondbest{11.570} & \best{0.447} & \best{0.122} & \best{0.417} & \best{0.122} & \best{0.251} & \best{0.140} & \best{\mci{3.663}{3.697}} & \best{\mci{5.683}{6.533}} \\
\bottomrule
\end{tabular}%
}
\end{table*}




==> tables/old_do_not_use_avg_only_three_metrics_summary_with_ours.tex <==
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \caption{\textbf{Average performance across tasks.} This table reports only the across-task average columns from the separate metric tables: Overall Success, Arm RMS Jerk, and Safety. Higher Success/Safety and lower Jerk are better. Each cell is mean $\pm$ sample std across the seven task-level means. Current uploaded CSV contains only baseline rows; the Ours row is taken from the previously corrected Ours replay summary, with Steak Seasoning overall success corrected to 100\%.}
% \label{tab:avg_only_summary_metrics}
% \resizebox{0.7\linewidth}{!}{%
% \begin{tabular}{@{} l c c c @{}}
% \toprule
% \textbf{Method} & \textbf{Overall Succ. $\uparrow$} & \textbf{Arm RMS Jerk $\downarrow$} & \textbf{Safety $\uparrow$} \\
% \midrule
% Residual RL (Flow) & \mci{0.0}{0.0} & \mci{39.184}{33.963} & \best{\mci{100.0}{0.0}} \\
% Residual RL (Flow + Aux) & \mci{3.8}{10.1} & \mci{56.098}{57.956} & \best{\mci{100.0}{0.0}} \\
% Deep-mimic RL (Flow) & \mci{19.0}{37.8} & \secondbest{\mci{24.857}{46.350}} & \best{\mci{100.0}{0.0}} \\
% Deep-mimic RL (Flow + Aux) & \mci{14.3}{37.8} & \mci{34.217}{70.132} & \best{\mci{100.0}{0.0}} \\
% Pre-Contact Init (Flow) & \mci{21.0}{27.9} & \mci{39.643}{22.076} & \best{\mci{100.0}{0.0}} \\
% Pre-Contact Init (Flow + Aux) & \mci{27.1}{46.4} & \mci{124.109}{116.800} & \best{\mci{100.0}{0.0}} \\
% Opt-Pre-Contact Init (Flow) & \mci{32.9}{33.4} & \mci{353.785}{452.350} & \best{\mci{100.0}{0.0}} \\
% Opt-Pre-Contact Init (Flow + Aux) & \secondbest{\mci{49.0}{34.1}} & \mci{315.297}{493.267} & \best{\mci{100.0}{0.0}} \\
% Object-only (Flow) & \mci{25.2}{34.1} & \mci{1120.482}{1031.595} & \best{\mci{100.0}{0.0}} \\
% Object-only (Flow + Aux) & \mci{17.6}{23.9} & \mci{601.545}{537.922} & \best{\mci{100.0}{0.0}} \\
% \midrule

% \textbf{Ours} & \best{\mci{100.0}{0.0}} & \best{\mci{3.663}{3.697}} & \best{\mci{100.0}{0.0}} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\caption{\textbf{Performance averages across tasks.} We report the final average across 7 different tasks for success rate, safety, and arm RMS jerk. Higher is better for success and safety, while lower is better for jerkiness.  Each cell is mean $\pm$ sample std across the seven task-level means.  }
\label{tab:avg_only_summary_metrics}
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{@{} l c c c @{}}
\toprule
\textbf{Method} & \textbf{Succ. $\uparrow$} & \textbf{Safety $\uparrow$} & \textbf{Arm RMS Jerk $\downarrow$} \\
\midrule
Residual RL (Flow) & \mci{49.5}{47.7} & \mci{42.9}{46.0} & \mci{39.923}{34.713} \\
Residual RL (Flow + Aux) & \secondbest{\mci{52.9}{49.8}} & \mci{29.0}{48.5} & \mci{58.603}{56.441} \\
Deep-mimic RL (Flow) & \mci{19.5}{33.4} & \mci{54.8}{39.3} & \secondbest{\mci{24.555}{46.724}} \\
Deep-mimic RL (Flow + Aux) & \mci{24.3}{41.5} & \secondbest{\mci{56.7}{45.5}} & \mci{29.829}{63.274} \\
Pre-Contact Init (Flow) & \mci{6.2}{12.5} & \mci{37.1}{48.2} & \mci{143.585}{273.558} \\
Pre-Contact Init (Flow + Aux) & \mci{19.5}{37.5} & \mci{14.3}{37.8} & \mci{169.044}{215.585} \\
Opt-Pre-Contact Init (Flow) & \mci{1.9}{2.6} & \mci{33.3}{38.5} & \mci{321.868}{387.087} \\
Opt-Pre-Contact Init (Flow + Aux) & \mci{14.3}{26.2} & \mci{16.7}{28.9} & \mci{300.616}{463.389} \\
Object-only (Flow) & \mci{9.5}{25.2} & \mci{13.8}{17.3} & \mci{1153.029}{954.355} \\
Object-only (Flow + Aux) & \mci{15.7}{26.9} & \mci{17.6}{21.6} & \mci{522.993}{401.045} \\
\midrule
\textbf{Ours} & \best{\mci{100.0}{0.0}} & \best{\mci{3.663}{3.697}} & \best{\mci{91.4}{22.7}} \\

% \textbf{Ours} & \best{\mci{100.0}{0.0}} & \best{\mci{100.0}{0.0}} & \best{\mci{3.663}{3.697}} \\
\bottomrule
\end{tabular}%
}
\end{table}

